Contextual Semantic Parsing for Multilingual Task-Oriented Dialogues

Robust state tracking for task-oriented dialogue systems currently remains restricted to a few popular languages. This paper shows that given a large-scale dialogue data set in one language, we can automatically produce an effective semantic parser for other languages using machine translation. We propose automatic translation of dialogue datasets with alignment to ensure faithful translation of slot values and eliminate costly human supervision used in previous benchmarks. We also propose a new contextual semantic parsing model, which encodes the formal slots and values, and only the last agent and user utterances. We show that the succinct representation reduces the compounding effect of translation errors, without harming the accuracy in practice. We evaluate our approach on several dialogue state tracking benchmarks. On RiSAWOZ, CrossWOZ, CrossWOZ-EN, and MultiWOZ-ZH datasets we improve the state of the art by 11%, 17%, 20%, and 0.3% in joint goal accuracy. We present a comprehensive error analysis for all three datasets showing erroneous annotations can lead to misguided judgments on the quality of the model. Finally, we present RiSAWOZ English and German datasets, created using our translation methodology. On these datasets, accuracy is within 11% of the original showing that high-accuracy multilingual dialogue datasets are possible without relying on expensive human annotations. We release our datasets and software open source.

==> model.tex <==
\section{Models}
\label{sec:model}

\subsection{CSP model}
Our CSP model is based on BART~\cite{}. The context is the previous gold slot-value pairs and last agent response. These are concatenated with current user utterance to form the input. The output is updated slot-value pairs. We use \textit{bart-base} and finetune it using token-level cross-entropy loss with teacher forcing. The model will learn to copy entities either from context or user utterance. As opposed to previous SOTA models~\cite{} which use separate modules to track and parse each part of the dialogue separately, our model encodes state, agent response, and user utterance as plain natural language in a unified manner.


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/model.pdf}
\caption{Contextual Semantic Parser model}
\label{fig:dialogue-loop}
\vspace{-1em}
\end{figure}


\subsection{Translation model}
We use MBART-50~\cite{} model for Chinese to English and Marian~\cite{} model for Chinese to Swedish translation. User and agent utterances are translated separately. We also translate all slot values in the ontology. Following the approach proposed in SPL, we first detect slot values in each conversation and preserve them during translation. This ensures there's no slot mismatches between natural language and annotations. It also allows different augmentation strategies for each data split to potentially create an open-ontology dialogue dataset where model encounter unseen slot values at test time. 

\subsection{Correction model}
To approximate human corrections, we finetuned a separate \textit{bart-base} model on a parallel dataset where the input is machine translated data and the output is human corrected translation. Since BART is pretrained with text denosing objective, this additional finetuning will direct it towards correcting lexical and syntactical mistakes machine translators make.
The dataset is constructed as follows:
First portion of the data comes from CrossWOZ (En). A quarter of the dev set has been selected and shown to professional human translators to correct the mistakes. We then align the machine translated examples with the human corrected examples.
Second portion of the data comes from MultiWOZ (Zh). We translate part of the dataset which is human translated back to English and align them with original English examples. 
